MixMOOD: A systematic approach to class distribution mismatch in semi-supervised learning using deep dataset dissimilarity measures

In this work, we propose MixMOOD - a systematic approach to mitigate effect of class distribution mismatch in semi-supervised deep learning (SSDL) with MixMatch. This work is divided into two components: (i) an extensive out of distribution (OOD) ablation test bed for SSDL and (ii) a quantitative unlabelled dataset selection heuristic referred to as MixMOOD. In the first part, we analyze the sensitivity of MixMatch accuracy under 90 different distribution mismatch scenarios across three multi-class classification tasks. These are designed to systematically understand how OOD unlabelled data affects MixMatch performance. In the second part, we propose an efficient and effective method, called deep dataset dissimilarity measures (DeDiMs), to compare labelled and unlabelled datasets. The proposed DeDiMs are quick to evaluate and model agnostic. They use the feature space of a generic Wide-ResNet and can be applied prior to learning. Our test results reveal that supposed semantic similarity between labelled and unlabelled data is not a good heuristic for unlabelled data selection. In contrast, strong correlation between MixMatch accuracy and the proposed DeDiMs allow us to quantitatively rank different unlabelled datasets ante hoc according to expected MixMatch accuracy. This is what we call MixMOOD. Furthermore, we argue that the MixMOOD approach can aid to standardize the evaluation of different semi-supervised learning techniques under real world scenarios involving out of distribution data.

==> images/FigureSSDL.tex <==
 
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100} 
\definecolor{mycolor2}{rgb}{0.92900,0.69400,0.12500} 
 
\begin{tikzpicture}
\centering
\begin{axis}[ 
width=5.521in,
height=2.06in,
at={(0.958in,0.481in)},
scale only axis,
xmin=-15,
xmax=15,
xtick={\empty},
ymin=-15,
ymax=15,
ytick={\empty},
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left
]
\addplot[only marks, mark=o, mark options={}, mark size=1.5000pt, draw=mycolor1] table[row sep=crcr]{ 
x	y\\
-2.50362744655278	3.77059752090627\\
3.35590411146651	-1.42658222054158\\
1.59157502867287	1.58706217326724\\
-0.409900570680579	-3.34354873811775\\
-1.98058576805972	-2.60289320004943\\
2.45234851291584	-4.25879155530057\\
-3.1600819535412	2.34845872866441\\
-0.00465771466283107	-4.16949962269386\\
2.16498481816524	-3.64924047406628\\
-1.29491456347496	2.6449151272755\\
-3.40301404789852	-1.15942050306958\\
3.69856785634583	-0.487813091570927\\
-1.88380268738714	-0.603048847809272\\
-1.81459983073475	3.2800348463609\\
-3.04761009290706	-2.84291310970322\\
-2.09134889408336	2.50751833412485\\
0.186961714284236	-4.56856715330964\\
-3.66546165982773	2.2020598253411\\
-2.99665985801667	0.14424197549878\\
-1.14658044121237	-3.1687004573112\\
3.06251496900158	-0.529858027631525\\
-2.06665687324927	3.888160930892\\
2.24559015142673	-3.64884947811824\\
-0.225016688274375	-3.27205036893565\\
3.99314948275832	-1.18261217721399\\
4.76364920721185	0.968495436148974\\
-2.75475531866993	3.46657440278631\\
-2.19098788317841	-3.58313669137003\\
-0.325102737335862	1.62100715553182\\
0.383861412060523	3.09853462869838\\
-0.92942210701387	-3.72944939731421\\
-2.40272104929848	-2.38986040563379\\
-0.944885595270367	-0.604723804992344\\
-1.27563610292553	-2.02236053497354\\
4.36435608475784	1.34429256185538\\
-0.36372343566112	0.508746085748133\\
-4.43130978657243	1.3986655074835\\
0.0797913421463607	1.39476150919408\\
-0.891022709555907	-3.99150889803524\\
2.1881085145909	-2.77803243958784\\
-0.459143117795165	2.28889330597457\\
-0.449019920557703	-3.75350159798082\\
1.13289433868028	1.33089413195478\\
2.12319652710226	-3.50302616776085\\
2.4939931597687	2.96135726012537\\
-1.00587766685134	-0.622586583556423\\
-0.791317502330605	0.884529295212528\\
0.681677979399751	-1.82970791588801\\
-0.700178483097923	-0.0166361337543568\\
-3.291344625896	0.215497554532064\\
3.26658205324103	-3.18354811044439\\
-2.37152654600562	3.13219030838529\\
-3.425592853301	1.12629879968934\\
4.5257505426504	-1.05559821856606\\
1.50796517591313	0.410474094516783\\
4.69598030482568	-0.805651324307567\\
0.612543921938978	1.5248630420843\\
-1.78868067154179	-3.11857987033785\\
-1.61957302948263	-0.977693077740583\\
-1.69536809893928	-3.33316536031055\\
-0.217351487054146	0.259323986083891\\
-3.18619067833561	-3.00253874693142\\
1.72660667723087	-4.27042855502803\\
4.75253575887512	0.577871626710234\\
4.29336564091378	2.4982430512287\\
3.50918918634016	-0.560284570056927\\
-1.51320157672128	-2.12032110743777\\
0.186659678287479	1.57604598998015\\
-2.92791380046219	2.03065052330564\\
2.75574389625971	2.65444979624296\\
-0.504825394466869	4.33789450296684\\
-0.0709696995582297	1.43841215564532\\
-1.99643852056103	3.54318191188202\\
2.07209264520339	2.93784060788691\\
-1.19444244360996	1.68804848480109\\
3.49635052954852	3.35253330823451\\
2.86847371844289	-2.55615687217485\\
2.75352387356986	1.85309829655683\\
4.39131400055646	-2.06502653888489\\
-3.2613353429618	2.40032024679558\\
3.21336174665173	0.986381780379675\\
-2.5124409821827	3.83145870773007\\
-0.321346560551213	-3.6348760570177\\
1.03103755042775	-3.57549132489366\\
-3.96026254334054	-1.14802388472449\\
-1.18187192074053	-2.78978966875628\\
1.91966416116057	-1.51563671874045\\
3.58112360480031	1.28399417390398\\
-1.54004403482844	4.39322668861988\\
3.05558443267743	0.912591244840766\\
0.56363967172428	1.58040781005559\\
-0.620774519190341	-3.27273355385035\\
-0.483648326914156	-2.6964225051391\\
2.27898659038147	-2.20020259663145\\
-3.96576638070891	-2.25981992644708\\
2.86842135374522	1.36487197447915\\
2.76242218115466	-1.4571966738673\\
0.934300898315582	-2.85277131328123\\
-0.419345293331521	1.82497493316944\\
-2.45478031420285	-0.690875141985264\\
1.46648554399875	-0.140704196414091\\
-0.701099856620799	-3.20053002144823\\
1.34504657934435	-2.15009751375154\\
-2.49112549532489	1.11048564615679\\
-3.20370371197354	0.598116057720099\\
-1.60222719880315	-0.642689263133884\\
-0.420998775824344	3.49276869056138\\
-0.0259166765285368	-4.20232185991467\\
-2.46692145944016	-0.0602729622419247\\
-2.67532878055485	-3.53119922466647\\
-0.483032553471162	1.27236746807292\\
2.01955156285978	2.40176958917649\\
-0.287871354573152	0.044532654579578\\
-1.52497498531034	1.78644160064172\\
0.0427696416512348	-0.175171274094608\\
0.411475419075952	-2.13545773883836\\
-0.924660006092586	-1.64532830877523\\
1.73018488663315	1.92571031989514\\
2.07185564658819	0.282339889309328\\
-1.73172424549571	-0.683633986411736\\
-1.21462726158416	3.67380196453391\\
4.40639794487295	-1.76354892007213\\
4.81123848411824	-0.580067578860965\\
-0.53630423220903	2.28953907347999\\
1.09045394942497	-3.29813501377579\\
2.43566792016355	-1.8622029107498\\
-2.96023563280963	-2.08122702327039\\
1.91970214164051	-1.71363897192366\\
1.22640816799963	-0.452607464846224\\
-3.14645962536801	-1.00397647528791\\
-0.28224348651945	-2.06559060523676\\
-0.715734710523402	-0.374701918896347\\
4.82104731769298	0.790227570119233\\
-3.09757092147439	1.08165030528434\\
-2.97326350355825	-3.89854696855124\\
-4.32713219522705	-0.579904358583693\\
-0.297920778984755	0.308155378048624\\
3.8057291126891	-1.58662910988489\\
2.01305336757736	-3.68732762248048\\
2.34183492253053	-3.26251879087324\\
-2.58650077430463	2.66791301530143\\
-1.94616603099691	-1.29040924685766\\
3.05903486031821	-3.15459364477963\\
2.18222091587695	-0.968824011015629\\
-1.4925860946715	-2.65401671515618\\
1.26601796309239	4.54647325327773\\
-2.62834742101207	-3.80804576228618\\
2.85235856072306	1.38740382960621\\
-2.34914454439645	1.55948640486244\\
-1.94475261775597	-3.38139365079046\\
4.3625710025977	-1.92947011240282\\
1.78139947158666	-4.42199848684425\\
-3.82764846945955	0.372783337784673\\
0.122240494531598	-2.88085793556111\\
-4.00488087651434	2.29946078357029\\
3.2735306592026	-0.586467688188994\\
4.74131424756152	-0.358923614880303\\
0.598629043114131	-0.686387949736478\\
-2.79474435597783	2.34522196118691\\
-4.06233821586026	1.18736762738876\\
0.0440662827337125	2.11674378663804\\
0.622475416203641	-2.83299267581981\\
1.60534641797013	-1.4545399935004\\
2.43009643421041	-1.46383431439865\\
-2.96678502933772	-1.13780682475223\\
-3.01140755765974	-2.15536122682346\\
0.655107989693865	0.888424640245828\\
3.00341881221245	-2.19038324681366\\
-2.49483137605472	0.803804407794864\\
0.675546614445736	2.36245218259835\\
1.99143874848577	-1.45354779632223\\
0.155079382505939	-1.95702238474\\
3.6163850278758	-3.29122596540504\\
-1.05356890697242	4.72033123267594\\
-2.09872078012957	-4.00789620839393\\
-2.18863028492109	-3.66284638928485\\
1.50265801669336	1.46195488704522\\
-2.50683198007864	1.6507779528805\\
-0.343721792810453	2.14513511117302\\
-0.0359840281123809	-0.169307621570598\\
-0.585646259918273	2.75091008605467\\
3.32376540980546	-2.5383081295436\\
1.82977959505256	-3.50475193672895\\
-2.83945329498063	2.348203434377\\
-3.31270654294605	0.0436514033469867\\
-0.911111437199545	-2.52102313279108\\
1.79061726954006	-3.05535062843729\\
-3.36846627722887	-2.77346166025656\\
-3.89322337730549	-1.97560445284977\\
-1.74496056448568	3.36994216060213\\
-4.16233978385712	1.16897325237286\\
-0.905981072324331	-3.91376557117606\\
1.31219576991579	-1.16560294248417\\
-0.646637164079519	-3.4916768006719\\
2.92631820440932	0.343794392891244\\
-0.690961794217786	-1.35139332507562\\
-1.78084159121826	0.724458368576258\\
-2.05809227480197	0.847643035163101\\
3.04021163642632	2.75024892367468\\
1.29839123118591	-3.01694543923599\\
-1.88819908259901	3.71413542652744\\
0.0600415927983717	2.53298422594534\\
-0.27173133609475	0.412466153900111\\
-2.59063854267609	2.56820340271625\\
-2.53061884345446	-0.762080967140206\\
-4.50024087896235	-1.84488099055586\\
-3.77644982841994	2.89819053137938\\
-2.51303139895811	1.87130638517679\\
-0.784605483350981	-0.075993957768866\\
-2.24872353712556	-3.4247864704079\\
4.3589996360554	-1.38866412688427\\
-0.85192737006356	-4.85404065845334\\
-0.96553331350629	0.700762125396888\\
1.65089140080158	-2.92107050601243\\
2.53543568086397	2.85189821901291\\
3.84774217624747	1.5364978058995\\
3.66055266661944	2.14153519462214\\
2.07604520849086	3.4555831766052\\
-1.91670500159727	3.80776912504793\\
-0.976202048713102	2.89710566015254\\
3.80281120511249	0.279605111885567\\
-1.6505324327835	-0.422735742296266\\
0.99138198268146	0.677141635691074\\
2.99601331508685	3.93929369496893\\
-1.81268077413903	-1.95825983530842\\
2.44566018774503	-2.98213073427689\\
4.84029778870851	-0.79091282193739\\
-1.94513196945239	-0.9278567813131\\
2.19638462993738	-0.043473633394442\\
-2.75869561163657	-0.964728530969027\\
-4.80657013458914	-0.468327809048062\\
-1.51728476766504	2.73213018526782\\
-2.36478421206115	1.11275034503946\\
-1.94643714651427	0.100296714006424\\
2.84215267457422	1.36010633518004\\
2.3303816293072	-1.98428403601112\\
1.66323491997927	0.715204360331138\\
-3.03631285714012	1.28717604893669\\
0.700448749709081	-1.34059715401244\\
-3.09029702564664	2.41158417717549\\
10.2512317526364	-5.75974518224942\\
14.4704927551454	-1.31856263472193\\
12.3950342661192	-6.49454072317135\\
0.200431567474076	-10.6329300012348\\
-9.43104447017362	-11.3185310763652\\
9.50655360749764	-9.71078998432405\\
-10.0691843405632	-9.27449755788862\\
13.7691617293246	-1.8562434866163\\
5.29722931539935	-13.347406531491\\
4.53059409801947	-13.9047601108896\\
-11.215485637579	-6.75728922114221\\
-10.9964139962471	-3.20774727056485\\
-9.9314927506826	-10.2654122887933\\
11.6302631274091	-5.53671639005698\\
14.0164582079399	-4.02125435213189\\
7.65753906830266	-10.5652398887783\\
9.45601169600431	-11.0587321992086\\
-9.07973693236588	-7.99909139121114\\
2.79248184952748	-11.4642448295953\\
12.16617047723	-8.23307326535374\\
-3.28742713125948	-10.5493995595854\\
14.1341014704626	-0.5135638619078\\
-13.7159157376182	-3.98478651457621\\
-7.0964406128766	-11.2556145226398\\
0.468771780199378	-13.0731518396086\\
-14.6787338007253	-2.82910868595646\\
8.56723384216778	-9.98715505070193\\
2.35372842682588	-13.1076778589417\\
1.10342663969085	-11.9290243744504\\
11.0644522740482	-6.54432310393439\\
11.5623127801253	-5.49597123776045\\
11.6105215506844	-9.06291074358198\\
-6.76144584067775	-10.4957125384921\\
-1.91268447320774	-12.6430692953404\\
9.39687680021678	-9.26624449461033\\
-13.3693418454279	-4.80669888772258\\
-11.1950131383788	-4.02022033037448\\
-9.70363474533156	-10.9985070908828\\
0.884720049136114	-11.4075822161822\\
13.3481440107006	-1.14969197199373\\
6.67431779107342	-8.58170469220611\\
-7.99047755717536	-11.9066959410047\\
-8.64172914713637	-11.2467833931507\\
10.979704256826	-5.57892170150484\\
13.5822622599997	-3.86989690553319\\
5.81878591020541	-12.4388940724244\\
-10.1561946915081	-10.5048054641374\\
-13.2073692143206	-3.77713845349062\\
12.8847175760327	-7.17566433749427\\
3.48199661264719	-12.7723853896717\\
12.8199336096499	-2.10863396793086\\
-13.2490800049948	-2.57181052398297\\
3.29261196912105	-12.0892704949265\\
-9.26196286453528	-11.5688678016313\\
11.4987494095731	-6.91138808659136\\
-10.3331572311404	-7.06931746475401\\
-2.38526861264699	-13.0674473438066\\
-4.66360690835516	-13.4026521352659\\
11.2644207308178	-6.82645957307562\\
6.3997198135663	-10.3069054085732\\
-11.6245331584199	-8.87751906104865\\
-7.47536557198278	-11.6257041704976\\
-11.9193172395539	-5.32826778748673\\
6.33761517688487	-10.6047841995941\\
2.72933514747643	-12.0342174624896\\
-11.7225923721455	-6.92114809503255\\
-11.8871479511508	-5.94694281502052\\
-1.07397381187824	-14.2645782289387\\
10.858327105997	-3.2249531603008\\
2.38283715508515	-14.4068087813449\\
-14.0471905894561	-1.45886694164668\\
-11.6790932411257	-1.99536356099445\\
11.9732466649013	-8.41138607491074\\
-1.86178416895902	-12.0926598853186\\
-5.00808952487988	-12.9628142775907\\
10.8035438447209	-8.3994732521916\\
-4.96864941739251	-10.9389295118139\\
1.05269516615201	-10.3223954773175\\
8.87984781281147	-11.3256195734389\\
13.2168616975954	-5.6468034100619\\
-6.78886895554547	-11.3722402795512\\
5.08465700761322	-9.9700605996817\\
13.7835221183676	-1.09192610761624\\
-11.7440128460415	-2.85726354498338\\
3.85214652416449	-13.7380831072343\\
-3.64917493524254	-13.1581158924132\\
-7.06268460315467	-10.3320176582448\\
-9.99261055119183	-10.9012491502752\\
10.4252481158922	-9.86627748650558\\
14.7074542025168	-0.221061423977004\\
-9.42343601595457	-6.25685331421543\\
9.38336538857224	-7.70589707693088\\
-11.6728853679874	-8.24763597158528\\
14.1693888704338	-0.340201439276796\\
11.7156720671045	-8.38540707014495\\
-3.1933578276168	-13.1603644931319\\
8.73442979540291	-9.97884135257594\\
-0.0719426441760875	-13.9088967338036\\
12.0702434943551	-8.25902288432937\\
-6.14091792874902	-12.6870508449621\\
};
\addplot[only marks, mark=diamond*, mark options={}, mark size=2.5883pt, color=red, fill=red] table[row sep=crcr]{ 
x	y\\
-3.09029702564664	2.41158417717549\\
-0.396289497477471	-0.342683442055998\\
1.58255870496812	-3.43904311210458\\
3.35569809104229	-2.9124794887551\\
2.20202698088787	-1.01747064046761\\
1.21665165064212	3.11773180334535\\
-0.203344952422198	3.76730744862265\\
0.992488496125218	-0.741621630166136\\
-2.93352293074992	-1.9497859769117\\
-4.00606221349803	-0.0966768132270211\\
-1.78545806631313	-1.5309417842018\\
};
\addplot[only marks, mark=o, mark options={}, mark size=1.5000pt, draw=mycolor2] table[row sep=crcr]{ 
x	y\\
4.61165998898138	12.7864757790238\\
3.85477110336962	13.8624753359381\\
0.213299279675244	11.5597002874813\\
1.89093068525109	10.8949123965717\\
3.52169812241684	11.6947783912386\\
3.64756522752323	11.0507281852178\\
1.12138535332257	12.5507625988263\\
1.34527365886683	14.5318216163261\\
3.36515582502059	13.1446196932616\\
2.38746098863431	10.5076694440616\\
3.11858206333721	11.9542737636318\\
1.18222466320455	10.2730830761183\\
0.885618772491583	12.5064145660161\\
4.14821692848792	12.1586058594212\\
3.83460833967632	14.9878017475609\\
4.67239136559135	14.0580129049766\\
0.539444525421818	12.4282583494901\\
0.911137528005279	14.472238777837\\
0.495476412112292	10.6877329738353\\
2.44881900961723	11.9500245722264\\
0.966226652344352	14.6367811249906\\
4.47945786896284	14.5874691620806\\
0.495448248409073	13.5678700579716\\
0.220827858813306	13.0916869181097\\
};
\addplot[only marks, mark=square*, mark options={}, mark size=1.0607pt, color=blue, fill=blue] table[row sep=crcr]{ 
x	y\\
-6.14091792874902	-12.6870508449621\\
-13.259058689717	-3.10593369831443\\
3.59051834900876	-12.2164878038095\\
13.6338410009165	-3.95227424586861\\
-10.7376407956954	-7.48451756560458\\
-2.90320582585821	-13.4576518932229\\
10.374976665149	-10.4298972698089\\
-14.4801997528723	-1.79159626151151\\
14.5311804024553	-2.4738122398203\\
10.9381676566183	-10.0366198233669\\
2.66700403057852	-14.2679506821351\\
};
\end{axis}
\end{tikzpicture} 

==> tables/half-half-results-v2.tex <==
\begin{table}
\caption{TBD}
\label{tab:half-half-results}
\begin{center}
\begin{small}

%l@{\qquad}c@{\;\;}c@{\qquad}c@{\;\;}c
\begin{tabular}{lccccccccc}
\toprule
 & \multicolumn{3}{c}{\textbf{MNIST}} 
 & \multicolumn{3}{c}{\textbf{CIFAR-10}}
 & \multicolumn{3}{c}{...} \\
 
   $N$ labelled 
 & 0 
 & 50 
 & 100
 & 0 
 & 50 
 & 100
 & 0 
 & 50 
 & 100 \\
 
 \midrule

   60 
 & $99\pm0.01$
 & $99\pm0.01$ 
 & $99\pm0.01$
 & $99\pm0.01$
 & $99\pm0.01$
 & $99\pm0.01$
 & $99\pm0.01$
 & $99\pm0.01$
 & $99\pm0.01$ \\
 
   100
 & $99\pm0.01$
 & $99\pm0.01$ 
 & $99\pm0.01$
 & $99\pm0.01$
 & $99\pm0.01$
 & $99\pm0.01$
 & $99\pm0.01$
 & $99\pm0.01$
 & $99\pm0.01$ \\
 
  150
 & $99\pm0.01$
 & $99\pm0.01$ 
 & $99\pm0.01$
 & $99\pm0.01$
 & $99\pm0.01$
 & $99\pm0.01$
 & $99\pm0.01$
 & $99\pm0.01$
 & $99\pm0.01$ \\
 
 \midrule
 Baseline
 & \multicolumn{3}{c}{$99\pm0.01$} 
 & \multicolumn{3}{c}{$99\pm0.01$}
 & \multicolumn{3}{c}{$99\pm0.01$}\\
 

 \bottomrule
\end{tabular}

\end{small}
\end{center}
\end{table}

==> tables/half-half-results.tex <==
\begin{table}
\caption{Results for OOD Type "Half-Half". Half-half means that the model only learns to predict on half of classes present in the data set. The data from the other half of classes is used as OOD data. OOD \% denotes the percentage of OOD data in the unlabeled data used for semi-supervised training. $N$ labelled denotes the number of labeled data points from the IOD data that were used during semi-supervised training. BL denotes a baseline, fully-supervised model that was trained on all labelled IOD data.}
\label{tab:half-half-results}
\begin{center}
\begin{small}

%l@{\qquad}c@{\;\;}c@{\qquad}c@{\;\;}c
\begin{tabular}{cc|ccc|c}
\toprule
 & & \multicolumn{3}{c|}{$N$ Labelled} & BL \\

Data Set & OOD \% & 60 & 100 & 150 & \\
\midrule
\multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{MNIST}}} & 60 & $00\pm0.00$ & $00\pm0.00$ & $00\pm0.00$ & \multirow{3}{*}{\textbf{$00\pm0.00$}} \\
 & 100 & $00\pm0.00$ & $00\pm0.00$ & $00\pm0.00$ & \\
 & 150 & $00\pm0.00$ & $00\pm0.00$ & $00\pm0.00$ & \\
\midrule
\multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{CIFAR}}} & 60 & $00\pm0.00$ & $00\pm0.00$ & $00\pm0.00$ & \multirow{3}{*}{\textbf{$00\pm0.00$}} \\
 & 100 & $00\pm0.00$ & $00\pm0.00$ & $00\pm0.00$ & \\
 & 150 & $00\pm0.00$ & $00\pm0.00$ & $00\pm0.00$ & \\
\midrule
\multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{...}}} & 60 & $00\pm0.00$ & $00\pm0.00$ & $00\pm0.00$ & \multirow{3}{*}{\textbf{$00\pm0.00$}} \\
 & 100 & $00\pm0.00$ & $00\pm0.00$ & $00\pm0.00$ & \\
 & 150 & $00\pm0.00$ & $00\pm0.00$ & $00\pm0.00$ & \\

 \bottomrule
\end{tabular}

\end{small}
\end{center}
\end{table}

==> tables/results-combined-June1-geneva1314.tex <==
\begin{table}
%\caption{\textbf{Results OOD Experiments.} IOD Data is the base data set that is considered IOD. OOD Type is the OOD configuration which can be \textit{half-half} (the model only learns to predict on half of the classes present in the data set while the data from the OH of classes is used as OOD data) or \textit{different} (data sets from a different data set than the IOD data are used as OOD data). OOD Data signifies the data set that was used as OOD data. OOD \% is the percentage of OOD data in the unlabeled data. $N$ Labelled is the number of labelled data points from IOD Data that were used during semi-supervised training. BL is the performance of a fully supervised baseline model trained on the entire data set of labelled IOD Data.}
\caption{$\mathbf{S_{IOD}}$: the dataset source used for the labelled data and the unlabelled IOD data, $\mathbf{T_{OOD}}$: type of unlabelled data used for the out of distribution setting (HH: half-half, Sim: human similar, Dif: human different), $\mathbf{S_{uOOD}}$: the dataset source used for the unlabelled OOD data (OH: other half, SVHN: Street View House Numbers, TI: Tiny ImageNet, G: Gaussian noise, SAP: Salt and pepper noise, FP: Fashion Product), $\mathbf{\%_{uOOD}}$: percentage of OOD data in the unlabelled data, $\mathbf{N_l}$: number of IOD labelled data points used in MixMatch training. Each result entry in the table represents the mean and variance of accuracy across ten random experimental runs per entry. For details about the runs please see the description in \Cref{sec:experiments}.}
\label{tab:half-half-results}
\begin{center}
\begin{small}


%l@{\qquad}c@{\;\;}c@{\qquad}c@{\;\;}c
\begin{tabular}{cccc|ccc}
\toprule
\multirow{2}{*}{$\mathbf{S_{IOD}}$} & \multirow{2}{*}{$\mathbf{T_{OOD}}$} & \multirow{2}{*}{$\mathbf{S_{uOOD}}$} & \multirow{2}{*}{$\mathbf{\%_{uOOD}}$} & \multicolumn{3}{c}{$\mathbf{N_l}$}\\

&  & &  & 60 & 100 & 150\\

\midrule

\multirow{12}{*}{\rotatebox[origin=c]{90}{\textbf{MNIST}}} 
& \multicolumn{3}{c|}{Fully supervised baseline} & $0.457\pm0.108$ & $0.559\pm 0.125 $ & $0.645 \pm0.101$ \\

 & \multicolumn{3}{c|}{SSDL baseline (no OOD data)} & $\mathbf{0.704 \pm 0.096}$ & $\mathbf{0.781\pm 0.065}$ & $\mathbf{0.831 \pm0.0626}$\\
 
 
 \cline{2-7}
 
 & \multirow{2}{*}{HH} & \multirow{2}{*}{OH} & 0 & $0.713\pm0.062$ & $0.802\pm0.064$ & $0.855\pm0.059$\\
 & & & 100 & $0.642 \pm 0.111$ & $0.746 \pm0.094$ & $0.798 \pm0.07$\\
 
 
 \cline{2-7}
 & \multirow{2}{*}{Sim} & \multirow{2}{*}{SVHN} & 50 & $0.637 \pm0.098$ & $0.745 \pm0.081$ & $0.801 \pm0.0699$\\
 
 & & & 100 & $0.482 \pm0.113$ & $0.719 \pm0.058$ & $0.765 \pm0.072$\\
 
  \cline{2-7}
 
  & \multirow{6}{*}{Dif}& \multirow{2}{*}{TI} & 50 & $0.642 \pm0.094$ & $0.739 \pm 0.074$ & $0.809 \pm0.066$\\
  
  & & & 100 & $0.637 \pm0.097$ & $0.732\pm 0.074$ & $0.804 \pm0.071$\\
  
  
 
 \cline{3-7}
 
  & & \multirow{2}{*}{G} & 50 & $0.606 \pm0.0989$ & $0.713 \pm0.087$ & $0.786\pm 0.065$\\
  
  & & & 100 & $0.442 \pm0.099$ & $0.461 \pm0.073$ & $0.542\pm 0.062$\\
  
 
  
   \cline{3-7}
 
  & & \multirow{2}{*}{SAP} & 50 & $0.631 \pm0.102$ & $0.735 \pm0.082$ & $0.813 \pm0.057$\\
  
  & & & 100 & $0.48\pm0.0951$ & $0.524 \pm0.09$ & $0.563 \pm0.095$\\
 
\midrule

\multirow{12}{*}{\rotatebox[origin=c]{90}{\textbf{CIFAR-10}}} & \multicolumn{3}{c|}{Fully supervised baseline} & $0.380\pm0.024$ & $0.445\pm0.042$ & $0.449\pm0.022$\\

 &  \multicolumn{3}{c|}{SSDL baseline (no OOD data)} & $\mathbf{0.453\pm0.046}$ & $0.474\pm0.019$ & $0.501\pm0.033$\\
 
 
 \cline{2-7}


& \multirow{2}{*}{HH} & \multirow{2}{*}{OH} & 50 & $0.444\pm0.040$ & $0.472\pm0.039$ & $0.525\pm0.050$\\ 
 & & & 100 & $0.443\pm0.023$ & $0.472\pm0.047$ & $0.499\pm0.054$ \\
 \cline{2-7}
 & \multirow{2}{*}{Sim} & \multirow{2}{*}{TI} & 50 & $0.435\pm0.054$ & $0.473\pm0.039$ & $\mathbf{0.543\pm0.040}$\\ 
 & & & 100 & $0.417\pm0.020$ & $\mathbf{0.480\pm0.039}$ & $0.498\pm0.042$ \\
 
 \cline{2-7}
 
  & \multirow{6}{*}{Dif} & \multirow{2}{*}{SVHN} & 50 & $0.419\pm0.027$ & $0.464\pm0.044$ & $0.469\pm0.056$\\ 
 & & & 100 & $0.385\pm0.034$ & $0.418\pm0.035$ & $0.440\pm0.046$ \\
 
 \cline{3-7}
 
  & & \multirow{2}{*}{G} & 50 & $0.409\pm0.047$ & $0.454\pm0.048$ & $0.491\pm0.032$\\ 
 & & & 100 & $0.297\pm0.029$ & $0.306\pm0.034$ & $0.302\pm0.038$ \\
 
 \cline{3-7}
 
  & & \multirow{2}{*}{SAP}& 50 & $0.438\pm0.029$ & $0.455\pm0.037$ & $0.485\pm0.034$\\ 
 & & & 100 & $0.236\pm0.031$ & $0.246\pm0.032$ & $0.232\pm0.022$ \\
  
  \midrule

\multirow{12}{*}{\rotatebox[origin=c]{90}{\textbf{FashionMNIST}}} & \multicolumn{3}{c|}{Fully supervised baseline} & $0.571\pm0.073$ & $0.704\pm0.066$ & $0.720\pm0.093$\\

 & \multicolumn{3}{c|}{SSDL baseline (no OOD data)} & $\mathbf{0.715\pm0.049}$ & $\mathbf{0.760\pm0.044}$ & $0.756\pm0.069$\\
 
 
 \cline{2-7}



& \multirow{2}{*}{HH} & \multirow{2}{*}{OH} & 50 & $0.714\pm0.049$ & $0.721\pm0.104$ & $0.765\pm0.053$\\ 
 & & & 100 & $0.660\pm0.061$ & $0.711\pm0.090$ & $0.747\pm0.061$ \\
 \cline{2-7}
 & \multirow{2}{*}{Sim} & \multirow{2}{*}{FP} & 50 & $0.707\pm0.039$ & $0.724\pm0.030$ & $0.778\pm0.078$\\ 
 & & & 100 & $0.546\pm0.101$ & $0.542\pm0.099$ & $0.540\pm0.105$ \\
 
 \cline{2-7}
 
  & \multirow{6}{*}{Dif}& \multirow{2}{*}{TI} & 50 & $0.690\pm0.065$ & $0.745\pm0.093$ & $0.792\pm0.058$\\ 
 & & & 100 & $0.690\pm0.073$ & $0.728\pm0.066$ & $\mathbf{0.794\pm0.056}$ \\
  
  \cline{3-7}
 
  & & \multirow{2}{*}{G} & 50 & $0.644\pm0.061$ & $0.689\pm0.075$ & $0.755\pm0.055$\\ 
 & & & 100 & $0.352\pm0.025$ & $0.366\pm0.065$ & $0.361\pm0.057$ \\
  
  \cline{3-7}
 
  & & \multirow{2}{*}{SAP} & 50 & $0.671\pm0.072$ & $0.708\pm0.095$ & $0.729\pm0.088$\\ 
 & & & 100 & $0.276\pm0.069$ & $0.297\pm0.046$ & $0.283\pm0.059$ \\
 
 \midrule

\multirow{12}{*}{\rotatebox[origin=c]{90}{\textbf{SVHN}}} & \multicolumn{3}{c|}{Fully supervised baseline} & $0.246\pm0.034$ & $0.253\pm0.021$ & $0.249\pm0.013$\\

 & \multicolumn{3}{c|}{SSDL baseline (no OOD data)} & $0.293\pm0.028$ & $0.332\pm0.050$ & $0.371\pm0.060$\\
 
 
 \cline{2-7}



& \multirow{2}{*}{HH} & \multirow{2}{*}{OH} & 50 & $0.307\pm0.048$ & $0.330\pm0.048$ & $0.380\pm0.048$\\ 
 & & & 100 & $0.307\pm0.053$ & $0.301\pm0.040$ & $0.398\pm0.055$ \\
 \cline{2-7}
 & \multirow{2}{*}{Sim} & \multirow{2}{*}{MNIST} & 50 & $0.296\pm0.040$ & $0.305\pm0.042$ & $0.293\pm0.043$\\ 
 & & & 100 & $0.287\pm0.040$ & $0.303\pm0.041$ & $0.274\pm0.028$ \\
 
 \cline{2-7}
 
  & \multirow{6}{*}{Dif} & \multirow{2}{*}{TI} & 50 & $\mathbf{0.339\pm0.047}$ & $0.361\pm0.048$ & $\mathbf{0.411\pm0.060}$\\ 
 & & & 100 & $0.323\pm0.056$ & $\mathbf{0.414\pm0.053}$ & $0.384\pm0.074$ \\
  
  \cline{3-7}
 
  & & \multirow{2}{*}{G} & 50 & $0.302\pm0.039$ & $0.360\pm0.040$ & $0.373\pm0.063$\\ 
 & & & 100 & $0.303\pm0.044$ & $0.284\pm0.050$ & $0.249\pm0.058$ \\
  
  \cline{3-7}
 
  & & \multirow{2}{*}{SAP} & 50 & $0.309\pm0.043$ & $0.332\pm0.033$ & $0.373\pm0.050$\\ 
 & & & 100 & $0.290\pm0.061$ & $0.294\pm0.070$ & $0.319\pm0.057$ \\


 \bottomrule
 
\end{tabular}

\end{small}
\end{center}
\end{table}
